M2QA: Multi-domain Multilingual Question Answering

Generalization and robustness to input variation are core desiderata of machine learning research. Language varies along several axes, most importantly, language instance (e.g. French) and domain (e.g. news). While adapting NLP models to new languages within a single domain, or to new domains within a single language, is widely studied, research in joint adaptation is hampered by the lack of evaluation datasets. This prevents the transfer of NLP systems from well-resourced languages and domains to non-dominant language-domain combinations. To address this gap, we introduce M2QA, a multi-domain multilingual question answering benchmark. M2QA includes 13,500 SQuAD 2.0-style question-answer instances in German, Turkish, and Chinese for the domains of product reviews, news, and creative writing. We use M2QA to explore cross-lingual cross-domain performance of fine-tuned models and state-of-the-art LLMs and investigate modular approaches to domain and language adaptation. We witness 1) considerable performance variations across domain-language combinations within model classes and 2) considerable performance drops between source and target language-domain combinations across all model sizes. We demonstrate that M2QA is far from solved, and new methods to effectively transfer both linguistic and domain-specific information are necessary. We make M2QA publicly available at https://github.com/UKPLab/m2qa.

==> Tables/chinese_results.tex <==
% \begin{table*}[]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{llcccccccccccc}
%         \toprule
%                     &           & \multicolumn{3}{c}{Creative Writing} & \multicolumn{3}{c}{Product Reviews}  & \multicolumn{3}{c}{News} & \multicolumn{3}{c}{Average}   \\
%          Model      &           & F1    & EM    & Acc                   & F1    & EM    & Acc                   & F1    & EM    & Acc       & F1    & EM    & Acc           \\
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          \XLMRBase  &  (0-shot)         & 13.00& 13.00& 59.73\%& 21.27& 21.20& 55.40\%& 45.88& 36.93& 61.33\%& 26.72& 23.71& 58.82\%\\
%          \XLMRDomain & (0-shot)         & 19.27& 19.27& 61.60\%& 28.31& 28.20& 52.40\%& 40.14& 39.73& 40.53\%& 29.24& 29.07& 51.51\%\\
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          MAD-X+Domain &  (0-shot)                       & 37.67& 37.67& 42.13\%& 37.19& 37.13& 46.27\%& 43.95& \textbf{39.40}& 56.20\%& 39.60& 38.07& 48.20\%\\
%          MAD-X$^2$  & (0-shot)               & 31.93& 31.93& 55.73\%& 35.13& 35.13& 49.73\%& \textbf{45.03}& 38.13& 57.53\%& 37.36& 35.06& 54.33\%\\

%          \midrule
%          Llama 2-chat (13b) &(0-shot) & 2.51& 0.00& 60.00\%& 1.63& 0.00& 60.00\%& 2.43& 0.00& 60.00\%& 2.19& 0.00& 60.00\%\\
%          gpt-35-turbo-0301 &(0-shot)& 39.07& 37.67& \textbf{70.93\%}& 33.92& 32.87& \textbf{71.40\%}& 30.14& 27.20& 75.47\%& 34.38& 32.58&\textbf{72.60\%} \\
%          gpt-3.5-turbo-0613 &(0-shot) & 47.79& 47.27& 69.93\%& 42.28& 41.73& 68.33\%& 39.85& 34.87& 76.33\%& 43.31& 41.29& 71.53\%\\
         
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          Llama 2-chat (13b)&(5-shot) & 38.56& 38.53& 45.27\%& 38.77& 38.67& 42.47\%& 39.43& 39.20& 42.60\%& 38.92& 38.80& 43.45\%\\
         
         
%          gpt-35-turbo-0301 &(5-shot)& 42.78& 41.00& 68.67\%& 38.75& 37.27& 69.13\%& 34.03& 30.73& 75.27\%& 38.52& 36.33&71.02\%\\
         
         
%          gpt-3.5-turbo-0613 &(5-shot) & \textbf{47.91}& \textbf{47.33}& 64.13\%& \textbf{43.48}& \textbf{42.73}& 64.40\%& 41.29& 37.00& 74.73\%& \textbf{44.23}& \textbf{42.35}& 67.75\%\\
         
         
%          \bottomrule
%     \end{tabular}
%     }
%     \caption{\textbf{Chinese} Results}
%     \label{tab:results_chinese}
% \end{table*}


\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llcccccccccccccc}
        \toprule
            &   & \multicolumn{3}{c}{Creative Writing} & \multicolumn{3}{c}{Product Reviews}  & \multicolumn{3}{c}{News} & \multicolumn{5}{c}{Average}   \\
                    &           & \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable & \multicolumn{2}{c}{Total Average}\\
         Model      &           & F1    & EM & F1   & F1    & EM & F1    & F1    & EM & F1    & F1    & EM & F1    & F1 & EM\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         \XLMRBase  &   (0-shot)        & 0.11& 0.11&                      32.33& 0.34& 0.22&                      52.67& 36.69& 21.78&          59.67& 12.38& 7.37&    48.22&  26.72&         23.71\\
         \XLMRDomain &     (0-shot)     & 0.00& 0.00&                      48.17& 0.41& 0.22&                      70.17& 1.02& 0.33&          98.83& 0.48& 0.18&    72.39&   29.24&        29.07\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         MAD-X+Domain &   (0-shot)  & 0.00&0.00&                      92.00&0.17&0.00&                          86.83&26.03&13.89&              66.17&8.73&4.63&  81.67&  39.60&   38.07\\
         MAD-X$^2$  & (0-shot) &0.11&0.11&   79.67& 0.00&0.00&      87.83&28.94&17.44&69.17&9.68&5.85&     78.89&   37.36&   35.06\\
         \midrule
         Llama 2-chat (13b) &(0-shot) &    &               &              &             &     &                  &       &        &        &       &       &   &     &   \\   
         gpt-35-turbo-0301 &(0-shot)& 27.12& 24.78& 57.00& 21.76& 20.00& 52.17& 16.56& 11.67& 50.50& 21.81& 18.82& 53.22& 34.38& 32.58\\
         gpt-3.5-turbo-0613 &(0-shot) & 35.31& 34.44& 66.50& 26.36& 25.44& 66.17& 26.86& 18.56& 59.33& 29.51& 26.15&  64.00&   43.31&      41.29\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         Llama 2-chat (13b) &(5-shot) &    0.71&               0.67&              95.33&             0.95&     0.78&                  95.50&       0.60&        0.22&        97.67&       0.75&       0.56&   96.17&     38.92&   38.80\\
         gpt-35-turbo-0301 &(5-shot)& 29.19& 26.22& 63.17& 27.59& 25.11& 55.50& 20.16& 14.67& 54.83& 25.65& 22.00&  57.83& 38.52&36.33\\
         gpt-3.5-turbo-0613 &(5-shot) & 29.30& 28.33& 75.83& 24.03&22.78& 72.67&23.59&16.44&67.83&25.64&22.52&    72.11&   44.23&    42.35\\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Chinese} Results}
    \label{tab:results_chinese}
\end{table*}

==> Tables/full_results_with_5shot.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllcccccccccccccc}
        \toprule
         &   &   & \multicolumn{3}{c}{\textbf{Creative Writing}} & \multicolumn{3}{c}{\textbf{Product Reviews}}  & \multicolumn{3}{c}{\textbf{News}} & \multicolumn{5}{c}{\textbf{Average}}   \\
                    & &           & \multicolumn{2}{c}{answerable} & unansrbl& \multicolumn{2}{c}{answerable} & unansrbl& \multicolumn{2}{c}{answerable} & unansrbl& \multicolumn{2}{c}{answerable} & unansrbl & \multicolumn{2}{c}{Total Average}\\
         & Model      &           & F1    & EM & F1   & F1    & EM & F1    & F1    & EM & F1    & F1    & EM & F1    & F1 & EM\\
         \midrule
         \multirow{10}{*}{\rotatebox[origin=l]{90}{\textbf{German}}} & \XLMRBase  &           & 30.42& 17.67&                      67.83& 35.64& 21.22&                      56.67& 40.98& 26.56&          55.33& 35.68& 21.82&    59.94&  45.38&         37.07\\
         & \XLMRDomain &        & 18.39& 9.44&                      79.00& 30.41& 17.00&                      60.83& 20.79& 11.56&          69.50& 23.20& 12.67&    69.78&   41.83&        35.51\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & MAD-X+Domain &    & 4.25&2.44& \textbf{94.83} &23.44&13.56&                          73.33&38.82&24.44&              55.33&22.17&13.48&  74.50&  43.19&   37.98\\
         & MAD-X$^2$  &  &19.09&11.33&   82.33& 22.96&13.44&      72.33&42.59&27.67&53.50&28.21&17.48&     69.39&   44.68&   38.24\\
         \cmidrule(lr){2-17}
         & Llama 2-chat (13b) &(0-shot) & 31.19 & 11.89 & 12.50 & 28.38& 11.00& 17.83& 39.33& 21.56& 12.83&       32.97&       14.82&   14.39&     25.53&   14.64\\   
         & gpt-3.5-turbo-0301 &(0-shot)& \textbf{40.49}& 20.67& 64.67& 45.31& 24.00& 61.17& 58.59& 36.22& 58.17& 48.13& 26.96& 61.34& 53.41& 40.71\\
         & gpt-3.5-turbo-0613 &(0-shot) & 37.68& 22.22& 80.50& 42.22& \textbf{24.44}& 76.50& 55.53& 37.67& 76.00& 45.14& 28.11&  77.67&   \textbf{58.15}&      47.93\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & Llama 2-chat (13b) &(5-shot) &    22.61&               12.33&              75.17&             20.52&     12.67&                  75.33&       29.33&        19.89&        \textbf{77.33}&       24.15&       14.96&   75.94&     44.87&   39.36\\
         & gpt-3.5-turbo-0301 &(5-shot)& 40.00& 21.89& 76.83& \textbf{47.81}& 24.33& 60.67& \textbf{61.18}& 38.22& 59.67& \textbf{49.66}& 28.15&  65.72& 56.09&43.18\\
         & gpt-3.5-turbo-0613 &(5-shot) & 34.97& \textbf{22.67}& 83.33& 40.36&23.33& \textbf{79.17}&58.50&\textbf{39.44}&70.83&44.61& \textbf{28.48}&    \textbf{77.78}&   57.88&    \textbf{48.20}\\
         
         \midrule
         \addlinespace
         \midrule
         
         \multirow{10}{*}{\rotatebox[origin=l]{90}{\textbf{Turkish}}} & \XLMRBase  &           & 22.65& 14.78&                      68.50& 32.68& 17.44&                      59.33& 41.71& 29.56&          57.17& 32.35& 20.59&    61.67&  44.08&         37.02\\
         & \XLMRDomain &          & 5.46& 3.22&                      89.33& 11.20& 5.11&                      77.83& 12.40& 6.67&          82.00& 9.69& 5.00&    83.05&   39.05&        36.22\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & MAD-X+Domain &     & 2.15&1.33& 96.00&11.33&6.00&                          90.33&30.97&20.78&              66.17&14.82&9.37&  84.17&  42.64&   39.04\\
         & MAD-X$^2$  &  &3.97&2.78& \textbf{97.17}& 8.43&4.89&      \textbf{93.17}&21.74&15.89&83.50&11.38&7.85& \textbf{91.28}&   43.34&   41.22\\
         \cmidrule(lr){2-17}
         & Llama 2-chat (13b) &(0-shot) & 18.11 &  9.00 & 5.00 & 22.16 & 9.22 & 6.00 & 22.27& 9.00& 4.83&       20.85&       9.07&   5.28&     14.62&   7.55\\   
         & gpt-3.5-turbo-0301 &(0-shot)& 36.58& 20.33& 68.33& 53.63& 25.00& 60.83& 53.67& 27.44& 54.50& 47.96& 24.26& 61.22& 53.26& 39.04\\
         & gpt-3.5-turbo-0613 &(0-shot) & \textbf{44.26}& \textbf{28.56}& 75.17& \textbf{57.29}& \textbf{32.33}& 63.67& 56.14& \textbf{33.78}& 57.67& \textbf{52.56}& \textbf{31.56}&  65.50&   \textbf{57.74}& \textbf{45.13}\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & Llama 2-chat (13b) &(5-shot) &    7.18&               5.22&              84.83&             8.48&     4.78&                  91.00&       9.78&        6.33&        \textbf{88.17}&       8.48&       5.44&   88.00&     40.29&   38.47\\
         & gpt-3.5-turbo-0301 &(5-shot)& 36.82& 22.78& 73.83& 53.89& 24.33& 61.67& \textbf{58.13}& 32.33& 55.00& 49.61& 26.48&  63.50& 55.17&41.29\\
         & gpt-3.5-turbo-0613 &(5-shot) & 33.58& 20.89& 84.50& 49.98&25.78& 71.17&55.21&32.00&58.00&46.26&26.22&    71.22&   56.24&    44.22\\
         
         \midrule
         \addlinespace
         \midrule
         
         \multirow{10}{*}{\rotatebox[origin=l]{90}{\textbf{Chinese}}} & \XLMRBase  &           & 0.11& 0.11&                      32.33& 0.69& 0.56&                      35.67& \textbf{39.67}& \textbf{24.44}&          49.33& 13.49& 8.37&    39.11&  23.74&         20.67\\
         & \XLMRDomain &         & 0.00& 0.00&                      48.17& 0.28& 0.22&                      62.33& 1.79& 1.00& \textbf{98.00}& 0.69& 0.41&    69.50&   28.21&        28.05\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & MAD-X+Domain &    & 0.00&0.00&                      92.00&0.39&0.33&                          85.00&32.21&20.22&              60.17&10.87&6.85&  79.06&  38.43&   36.02\\
         & MAD-X$^2$  & &0.11&0.11&   79.67& 0.17&0.11&      83.67&33.24&22.00&68.67&11.17&7.41&     77.34&   37.64&   35.38\\
         \cmidrule(lr){2-17}
         & Llama 2-chat (13b) &(0-shot) & 13.05 & 2.44 & 16.17 & 12.39& 3.89& 17.50&     10.86& 1.89& 14.67&       12.10& 2.74&  16.11&  13.70& 8.09\\   
         & gpt-3.5-turbo-0301 &(0-shot)& 27.12& 24.78& 57.00& 19.50& 16.56& 60.50& 18.86& 15.00& 43.50& 21.83& 18.78& 53.67& 34.56& 32.73\\
         & gpt-3.5-turbo-0613 &(0-shot) & \textbf{35.31}& \textbf{34.44}& 66.50& \textbf{26.01}& \textbf{25.44}& 71.67& 27.88& 21.78& 53.83& \textbf{29.73}& \textbf{27.22}&  64.00&   \textbf{43.44}&      \textbf{41.93}\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-17}
         & Llama 2-chat (13b) &(5-shot) &    0.71&               0.67& \textbf{95.33}&             1.50&     1.44& \textbf{90.83}&       1.19&        0.78&        96.00&       1.13&       0.96&   \textbf{94.05}&     38.30&   38.20\\
         & gpt-3.5-turbo-0301 &(5-shot)& 29.19& 26.22& 63.17& 21.05& 16.89& 63.67& 21.55& 17.33& 48.50& 23.93& 20.15&  58.45& 37.74&35.47\\
         & gpt-3.5-turbo-0613 &(5-shot) & 29.30& 28.33& 75.83& 16.07&14.67& 82.33&25.44&20.11&57.83&23.60&21.04&    72.00&   42.96&    41.42\\
         \bottomrule

    \end{tabular}
    }
    % \vspace{-2mm}
    \vspace{-2.5mm}
    \caption{Results of the base models and adapter-based methods on the M2QA benchmark using the F1/EM score definitions by SQuAD 2.0 \cite{rajpurkar-etal-2018-know}.
    See our discussion of this metric's potential flaws in Section \ref{sec:ablation:squad_metric_multilingual}.
    For the answerable questions, we report the F1 and Exact Match (EM) scores. For the unanswerable (unansrbl) questions, we only include the F1 score as the EM score is identical to it by definition. The average is taken across datapoints.
    The best score for each language in each column is bold.}
    % \vspace{-4.5mm}
    \vspace{-5.5mm}
    \label{tab:full_results}
\end{table*}


==> Tables/german_results.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll|ccc|ccc|ccc|ccc}
        \toprule
                    &           & \multicolumn{3}{c|}{Creative Writing} & \multicolumn{3}{c|}{Product Reviews}  & \multicolumn{3}{c|}{News} & \multicolumn{3}{c}{Average}   \\
         model      &           & F1    & EM    & Acc                   & F1    & EM    & Acc                   & F1    & EM    & Acc       & F1    & EM    & Acc           \\
         \midrule
         \XLMRBase  &           & 45.38 & 37.73 &                       58.80\%& 44.58 & 35.93 &                       60.20\%& 47.46 & 40.33 &           62.07\%& 45.81 & 38.00 &               60.36\%\\
         \XLMRDomain &          & 42.64 & 37.27 &                       52.93\%& 42.20 & 34.27 &                       59.07\%& 42.17 & 37.67 &           54.07\%& 42.34 & 36.40 &               55.36\%\\
         \midrule
         Llama 2-chat &(zero-shot) &    6.57&       0.00&                       60.00\%&       5.95&       0.00&                       60.00\%&       7.19&       0.00&           60.00\%&       6.57&       0.00&           60.00\%\\
         Llama 2-chat &(five-shot) &    43.63&       37.47&                       59.47\%&       44.40&       39.73&                       59.80\%&       49.50&       44.93&           62.33\%&       45.84&       40.71&           60.53\%\\
         \hdashline
         gpt-35-turbo-0301 &(zero-shot)& 50.16& 38.27& \textbf{72.47\%}& 55.16& 40.93& 77.73\%& 55.88& 42.07& 76.60\%& 53.73& 40.42&\textbf{75.60\%} \\
         gpt-35-turbo-0301 &(five-shot)& 54.74& 43.87&  70.40\%& 55.34& 40.53& \textbf{77.93\%}& 57.17& 43.20& 75.93\%& 55.75& 42.53&74.75\%\\
         \hdashline
         gpt-3.5-turbo-0613 &(zero-shot) & \textbf{54.81} & 45.53 &              69.00\%& \textbf{59.68} & \textbf{48.93} &                       77.47\%& 62.10 & 51.07 &           \textbf{79.67\%}& \textbf{58.86} & 48.51 &           75.38\%\\
         gpt-3.5-turbo-0613 &(five-shot) & 54.32 & \textbf{46.93} &              66.20\%& 58.41&47.40&                          75.27\%&\textbf{62.72}&\textbf{51.67}&               79.33\%&58.48&\textbf{48.67}    &           73.60\%\\
         \midrule
         MAD-X+Domain &     & 40.75 &39.67      &                       42.67\%&44.82&40.87&                           55.20\%&47.85&42.67&               59.13\%&44.47&41.07    &       52.33\%\\
         MAD-X$^2$  &(250k steps)&44.39&39.73&                         52.47\%&44.18&37.73&                           55.00\%&44.84&36.53&               61.60\%&44.47&38.00     &           56.36\%\\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{German} Results}
    \label{tab:results_german}
\end{table*}

==> Tables/turkish_results.tex <==
% \begin{table*}[]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{llcccccccccccc}
%         \toprule
%                     &           & \multicolumn{3}{c}{Creative Writing} & \multicolumn{3}{c}{Product Reviews}  & \multicolumn{3}{c}{News} & \multicolumn{3}{c}{Average}   \\
%          model      &           & F1    & EM    & Acc                   & F1    & EM    & Acc                   & F1    & EM    & Acc       & F1    & EM    & Acc           \\
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          \XLMRBase  &   (0-shot)        & 40.99& 36.27& 52.73\%& 43.34& 34.20& 60.53\%& 46.72& 38.47& 60.33\%& 43.68& 36.31& 57.86\%\\
%          \XLMRDomain &  (0-shot)        & 39.01 & 37.67& 44.73\%& 37.86& 34.20& 49.00\%& 39.27& 35.93& 49.87\%& 38.71& 35.93& 47.87\%\\
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          MAD-X+Domain &   (0-shot)                      & 39.95& 38.87& 41.13\%& 42.92& 39.33& 47.20\%& 48.39& 43.00& 58.93\%& 43.75& 40.40& 49.09\%\\
%          MAD-X$^2$  &(0-shot)               & 41.25& 40.53& 42.13\%& 42.32& 40.20& 45.20\%& 46.45& 42.73& 53.27\%& 43.34& 41.15& 46.87\%\\
%          \midrule
%          Llama 2-chat &(0-shot) & 3.13& 0.00& 60.00\%& 4.27& 0.00& 60.00\%& 5.15& 0.00& 60.00\%& 4.18& 0.00& 60.00\%\\
%          gpt-35-turbo-0301 &(0-shot)& 49.28& 39.53& 74.80\%& 56.51& 39.33& \textbf{79.73\%}& 57.27& 40.53& 80.93\%& 54.35& 39.80&78.49\%\\
%          gpt-3.5-turbo-0613 &(0-shot) & \textbf{56.62}& \textbf{47.20}& \textbf{75.87\%}& \textbf{59.84}& \textbf{44.87}& \textbf{79.73\%}& \textbf{61.16}& \textbf{46.73}& \textbf{81.80\%}& \textbf{59.21}& \textbf{46.27}& \textbf{79.13\%} \\
         
         
         
%          \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%          Llama 2-chat &(5-shot) & 38.24& 37.07& 43.20\%& 41.49& 39.27& 45.93\%& 41.31& 39.20& 46.33\%& 40.35& 38.51& 45.15\%\\
%          gpt-35-turbo-0301 &(5-shot)& 51.62& 43.20& 71.87\%& 57.00& 39.27& 79.00\%& 59.63& 43.60& 81.33\%& 56.08& 42.02&77.40\%\\
         
%          gpt-3.5-turbo-0613 &(5-shot) & 53.95& 46.33& 68.20\%& 58.46& 43.93& 75.67\%& 60.64& 45.40& 81.53\%& 57.68& 45.22& 75.13\%\\
        
         
         
%          \bottomrule
%     \end{tabular}
%     }
%     \caption{\textbf{Turkish} Results}
%     \label{tab:results_turkish}
% \end{table*}

\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llcccccccccccccc}
        \toprule
            &   & \multicolumn{3}{c}{Creative Writing} & \multicolumn{3}{c}{Product Reviews}  & \multicolumn{3}{c}{News} & \multicolumn{5}{c}{Average}   \\
                    &           & \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable& \multicolumn{2}{c}{answerable} & unanswerable & \multicolumn{2}{c}{Total Average}\\
         Model      &           & F1    & EM & F1   & F1    & EM & F1    & F1    & EM & F1    & F1    & EM & F1    & F1 & EM\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         \XLMRBase  &   (0-shot)        & 22.65& 14.78&                      68.50& 32.68& 17.44&                      59.33& 42.86& 29.11&          52.50& 32.73& 20.44&    60.11&  43.68&         36.31\\
         \XLMRDomain &     (0-shot)     & 5.46& 3.22&                      89.33& 11.20& 5.11&                      77.83& 14.34& 8.78&          77.00& 10.33& 5.70&    81.39&   38.71&        35.93\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         MAD-X+Domain &   (0-shot)  & 2.15&1.33&                      96.00&11.33&6.00&                          90.33&33.35&22.00&              62.83&15.61&9.78&  83.05&  43.75&   40.40\\
         MAD-X$^2$  & (0-shot) &3.97&2.78&   97.17& 8.43&4.89&      93.17&22.75&16.56&82.00&11.72&8.08&     90.78&   43.34&   41.15\\
         \midrule
         Llama 2-chat (13b) &(0-shot) &    &               &              &             &     &                  &       &        &        &       &       &   &     &   \\   
         gpt-35-turbo-0301 &(0-shot)& 36.58& 20.33& 68.33& 53.63& 25.00& 60.83& 54.55& 26.67& 61.33& 48.25& 24.00& 63.50& 54.35& 39.80\\
         gpt-3.5-turbo-0613 &(0-shot) & 44.26& 28.56& 75.17& 57.29& 32.33& 63.67& 56.38& 32.33& 68.33& 52.64& 31.07&  69.06&   59.21&      46.27\\
         \cmidrule(lr){1-2}\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16}
         Llama 2-chat (13b) &(5-shot) &    7.18&               5.22&              84.83&             8.48&     4.78&                  91.00&       8.52&        5.00&        90.50&       8.06&       5.00&   88.78&     40.35&   38.51\\
         gpt-35-turbo-0301 &(5-shot)& 36.82& 22.78& 73.83& 53.89& 24.33& 61.67& 57.83& 31.11& 62.33& 49.51& 26.07&  65.94& 56.08&42.02\\
         gpt-3.5-turbo-0613 &(5-shot) & 33.58& 20.89& 84.50& 49.98&25.78& 71.17&56.84&31.44&66.33&46.80&26.04&    74.00&   57.68&    45.22\\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Turkish} Results}
    \label{tab:results_turkish}
\end{table*}
